SVT: Supertoken Video Transformer for Efficient Video Understanding

Whether by processing videos with fixed resolution from start to end or incorporating pooling and down-scaling strategies, existing video transformers process the whole video content throughout the network without specially handling the large portions of redundant information. In this paper, we present a Supertoken Video Transformer (SVT) that incorporates a Semantic Pooling Module (SPM) to aggregate latent representations along the depth of visual transformer based on their semantics, and thus, reduces redundancy inherent in video inputs.~Qualitative results show that our method can effectively reduce redundancy by merging latent representations with similar semantics and thus increase the proportion of salient information for downstream tasks.~Quantitatively, our method improves the performance of both ViT and MViT while requiring significantly less computations on the Kinectics and Something-Something-V2 benchmarks.~More specifically, with our SPM, we improve the accuracy of MAE-pretrained ViT-B and ViT-L by 1.5% with 33% less GFLOPs and by 0.2% with 55% less FLOPs, respectively, on the Kinectics-400 benchmark, and improve the accuracy of MViTv2-B by 0.2% and 0.3% with 22% less GFLOPs on Kinectics-400 and Something-Something-V2, respectively.

==> _tables.tex <==
% \begin{table}
%   \centering
%   \resizebox{1.0\linewidth}{!}{
%   \begin{tabular}{@{}lccc@{}}
%       \toprule
%       model & layer & $T_w \times H_w \times W_w$ & $N_{win}\times M+N_k=N_r$ \\
%       \midrule
%       B-SPM6 & 6 & 2x14x14 & 4$\times$32+0=128 \\
%       B-SPM8 & 8 & 2x14x14 & 4$\times$32+0=128 \\
%       \midrule
%       L-SPM12 & 12 & 2x14x14 & 4$\times$32+0=128 \\
%       L-SPM16 & 16 & 2x14x14 & 4$\times$32+0=128 \\
%       L-SPM18 & 16 & global & 1$\times$64+0=64 \\
%       \midrule
%       \multirow{3}{*}{L-SPM8/12/16} & 8 & 2x14x14 & 4$\times$32+896=1024 \\
%                                           & 12 & global & 1$\times$128+384=512 \\
%                                           & 16 & global & 1$\times$128+0=128 \\
%       \midrule
%       \multirow{3}{*}{L-SPM8/14/18} & 8 & 2x14x14 & 4$\times$32+896=1024 \\
%                                           & 14 & global & 1$\times$128+384=512 \\
%                                           & 18 & global & 1$\times$128+0=128 \\
%       \bottomrule
%   \end{tabular}
%   }
%   \caption{config.}
%   \label{tab:config}
% \end{table}


% \begin{table}
%   \centering
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     Model & Acc & \#Params(M) & GFLOPs \\
%     \midrule
%     MAE-ViT-B & 83.6 & 86 & 18 \\
%     \rowcolor{gray!20}ours-B-SPM8 & - & 86 & 12 \\
%     \midrule
%     MAE-ViT-L & 85.9 & 304 & 62 \\
%     ToMe-ViT-L & 84.2 & 304 & 22 \\
%     ToMe-ViT-L & 85.1 & 304 & 31 \\
%     \rowcolor{gray!20}ours-L-SPM16 & \textbf{85.8} & 304 & 43 \\
%     \midrule
%     MAE-ViT-H & 86.9 & 632 & 167 \\
%     ToMe-ViT-H & 86.1 & 632 & 73 \\
%     ToMe-ViT-H & 86.5 & 632 & 92 \\
%     \rowcolor{gray!20}ours-H-SPM22 & \textbf{86.9} & 632 & 123 \\
%     \midrule
%     \midrule
%     MViT-v2-T & 82.3 & 24 & 4.7 \\
%     \rowcolor{gray!20}ours-T & 81.3 & 24 & 3.8 \\
%     \midrule
%     MViT-v1-B-16 & 83.0 & 37 & 7.8 \\
%     MViT-v2-S & 83.6 & 35 & 7.0 \\
%     \rowcolor{gray!20}ours-S & 82.7 & 35 & 6.0 \\
%     \midrule
%     MViTv1-B-24 & 83.4 & 54 & 10.9 \\
%     MViT-v2-B & 84.4 & 52 & 10.2 \\
%     \rowcolor{gray!20}ours-B & 83.7 & 52 & 8.8 \\
%     \bottomrule
%   \end{tabular}
%   \caption{IN1k.}
%   \label{tab:in1k}
% \end{table}

% \begin{table}
% \centering
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{lcccc}
%   \toprule
%   model & top-1 & top-5 & GFLOPs & \#Params/M \\
%   \midrule
%   MAE-ViT-B & 79.3 & 93.2 & 180$\times$3$\times$7 & 87 \\
%   \rowcolor{gray!20}ours-B-SPM6 & \textbf{79.9} & \textbf{94.5} & 91$\times$3$\times$7 & 87 \\
%   \rowcolor{gray!20}ours-B-SPM8 & \textbf{80.8} & \textbf{94.8} & 120$\times$3$\times$7 & 87 \\
%   \midrule

%   MAE-ViT-L & 84.8 & 96.2 & 598$\times$3$\times$7 & 304 \\
%   ToMe-ViT-L\cite{bolya2022token} & 83.2 & - & 184$\times$1$\times$10 & 304 \\
%   ToMe-ViT-L\cite{bolya2022token} & 84.4 & - & 281$\times$1$\times$10 & 304 \\
%   \rowcolor{gray!20}ours-L-SPM12 & 84.6 & 96.2 & 302$\times$3$\times$7 & 304 \\
%   \rowcolor{gray!20}ours-L-SPM16 & \textbf{85.0} & \textbf{96.6} & 473$\times$3$\times$7 & 304 \\
%   \rowcolor{blue!10}ours-L-SPM18 & \textbf{85.1} & \textbf{96.5} & 509$\times$3$\times$7 & 304 \\
%   \rowcolor{gray!20}ours-L-SPM8/12/16 & \textbf{84.8} & \textbf{96.4} & 254$\times$3$\times$7 & 304 \\
%   \rowcolor{blue!10}ours-L-SPM8/14/18 & \textbf{85.0} & \textbf{96.5} & 275$\times$3$\times$7 & 304 \\
%   \midrule
%   MAE-ViT-H & 85.1 & 96.6 & 1193$\times$3$\times$7 & 632 \\
%   \rowcolor{gray!20}ours-H-SPM22 & \textbf{85.1} & \textbf{96.7} & - & 632 \\
%   \rowcolor{gray!20}ours-H-SPM12/18/24 & - & - & - & 632 \\
%   \midrule
%   \midrule
%   MViTv1, 16x4 & 78.4 & 93.5 & 70$\times$1$\times$5 & 37 \\
%   MViTv2-S, 16x4 & 81.0 & 94.6 & 64$\times$1$\times$5 & 34 \\
%   \rowcolor{gray!20}ours-S, 16x4 & 80.9 & 94.6 & 59$\times$1$\times$5 & 34 \\
%   \midrule
%   MViTv1, 32x3 & 80.2 & 94.4 & 170$\times$1$\times$5 & 37 \\
%   MViTv2-B, 32x3 & 82.9 & 95.7 & 225$\times$1$\times$5 & 51 \\
%   \rowcolor{gray!20}ours-B, 32x3 & \textbf{83.0} & 95.6 & 176$\times$1$\times$5 & 51 \\
%   \bottomrule
% \end{tabular}
% }
% \caption{K400.}
% \label{tab:k400}
% \end{table}



% \begin{table}
% \centering
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{lcccc}
%   \toprule
%   model & top-1 & top-5 & GFLOPs & \#Params/M \\
%   \midrule
%   MAE-ViT-L & 72.1 & 93.9 & 598$\times$3$\times$1 & 304 \\
%   \rowcolor{gray!20}ours-L-SPM16 & 71.7 & 93.8 & 473$\times$3$\times$1 & 304 \\
%   \rowcolor{gray!20}ours-L-SPM18 & - & - & 509$\times$3$\times$1 & 304 \\
%   \rowcolor{gray!20}ours-L-SPM8/14/18 & - & - & 275$\times$3$\times$1 & 304 \\
%   \midrule
%   MAE-ViT-H & 74.1 & 94.5 & 1193$\times$3$\times$1 & 632 \\
%   \rowcolor{gray!20}ours-H-SPM22 & - & - & - & 632 \\
%   \rowcolor{gray!20}ours-H-SPM12/18/24 & - & - & - & 632 \\
%   \midrule
%   \midrule
%   MViTv1, 16x4 & 64.7 & 89.2 & 71$\times$1$\times$5 & 37 \\
%   MViTv2-S, 16x4 & 68.2 & 91.4 & 64$\times$1$\times$5 & 34 \\
%   \rowcolor{gray!20}ours-S, 16x4 & 68.0 & 91.0 & 53$\times$1$\times$5 & 34 \\
%   \midrule
%   MViTv1, 64x3 & 67.7 & 90.9 & 454$\times$1$\times$5 & 37 \\
%   MViTv2-B, 32x3 & 70.5 & 92.7 & 225$\times$1$\times$5 & - \\
%   \rowcolor{gray!20}ours-B, 32x3 & - & - & 176$\times$1$\times$5 & 51 \\
%   \bottomrule
% \end{tabular}
% }
% \caption{SSV2.}
% \label{tab:ssv2}
% \end{table}


==> _todo.tex <==
memory requirements

